A+ Indexes: Tunable and Space-Efficient Adjacency Lists in Graph Database Management Systems

Graph database management systems (GDBMSs) are highly optimized to perform fast traversals, i.e., joins of vertices with their neighbours, by indexing the neighbourhoods of vertices in adjacency lists. However, existing GDBMSs have system-specific and fixed adjacency list structures, which makes each system efficient on only a fixed set of workloads. We describe a new tunable indexing subsystem for GDBMSs, we call A+ indexes, with materialized view support. The subsystem consists of two types of indexes: (i) vertex-partitioned indexes that partition 1-hop materialized views into adjacency lists on either the source or destination vertex IDs; and (ii) edge-partitioned indexes that partition 2-hop views into adjacency lists on one of the edge IDs. As in existing GDBMSs, a system by default requires one forward and one backward vertex-partitioned index, which we call the primary A+ index. Users can tune the primary index or secondary indexes by adding nested partitioning and sorting criteria. Our secondary indexes are space-efficient and use a technique we call offset lists. Our indexing subsystem allows a wider range of applications to benefit from GDBMSs' fast join capabilities. We demonstrate the tunability and space efficiency of A+ indexes through extensive experiments on three workloads.

==> eb-vs-vb-experiment-tables.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{justification=centering}
	\begin{tabular}{m{1.55cm} % dataset - sys.
		m{1.65cm} m{1.65cm} m{1.65cm}} % m{1.65cm} m{1.65cm}}
		\toprule
		selectivity & 25\% & 5\% & 0.05\% \\ %& 1\% \\ 10\% & 0.2\% \\
	    \midrule
		\texttt{D}\newline
		\texttt{D+EP$_c$}
		& 1028.8 \newline 61.66~\textbf{(16.7x)}
		%10\%  & 1024.8 \newline 53.11~\textbf{(19.3x)}
		& 1047.5 \newline 47.77~\textbf{(21.9x)}
		%1\%   & 1019.3 \newline 40.54~\textbf{(25.1x)}
		%0.2\% & 1032.0 \newline 35.23~\textbf{(29.3x)}
		& 1056.3 \newline 29.71~\textbf{(35.6x)}  \\
		\midrule
		Mm(\texttt{D+EP$_c$})\newline
		|E$_{indexed}$|
		& 5558~\textbf{(3.45x)} \newline 1.466 B
		%10\%  & 3809~\textbf{(2.36x)} \newline 587.3 M
		& 3116~\textbf{(1.93x)} \newline 276.2 M
		%1\%   & 2452~\textbf{(1.50x)} \newline 69.6 M
		%0.2\% & 2061~\textbf{(1.28x)} \newline 11.7 M
		& 1951~\textbf{(1.21x)} \newline 2.9 M \\
		\bottomrule
	\end{tabular}
	%\vspace{-8pt}
	\caption{Runtime (in secs) for a 2-hop MoneyFlow query on LJ using index configurations \texttt{D} and \texttt{D+EP$_c$} introduced in Section~\ref{sec:secondary-edge-bound-eval}. We report the number of indexed edges and memory (Mm) of \texttt{D+EP$_c$} and compare it to \texttt{D} of size 1612 MB.}
	\label{tab:eb-vs-eb-runtime}
	\vspace{-19pt}
\end{table}


==> overview-aplus-indexes.tex <==
\vspace{-4pt}
\subsection{Overview of A+ Indexes}

Our indexing subsystem contains three types of indexes.

\noindent {\bf Primary A+ Indexes:} Instead of a system-specific fixed criteria, users can provide arbitrary nested partitioning and sorting on the system's primary adjacency lists. The edges are then indexed in a nested CSR-like data structure that has as many levels as there are partitioning criteria. The most granular lists are then sorted according to the given sorting criteria. Figure~\ref{fig:global-view} shows an example primary A+ index on our running example that 
has two nested partitioning levels on top of the primary vertex ID partitioning: (i) by edge labels; and (ii) by \texttt{currency} property.  This allows the system to provide fast joins for workloads that access edges that satisfy other equality predicates without data remodelling and with no or negligible memory costs.%, leading to significant performance gains in some settings. 

\noindent {\bf Secondary A+ Indexes:}
We observe that each partitioning level of existing indexes identifies
a sublist, which is a view over edges that satisfy a set of equality predicates. Figure~\ref{fig:global-view} shows the nested sublists with different types of boxes. For example, the blue dashed box corresponds to view $\sigma_{\text{srcID=v1}}$\texttt{E}, while the red dash-dotted box corresponds to  $\sigma_{\text{srcID=v1 \& e.label=Wire}}$\texttt{E}, where \texttt{E} is the set of all edges.  Therefore query processors of existing systems effectively evaluate queries using views when they probe adjacency list indexes to access these lists. 
One can also think of the entire adjacency list index as partitioning one {\em global view} into lists, which in 
Figure~\ref{fig:global-view} is simply the set of edges, shown in a solid grey box. 
To support access to a larger set of views, we first allow users to define two other types of global views that are indexed in our {\em secondary A+ indexes}. Our choice of the views we support allows us to provide a space-efficient implementation with an appropriate partitioning, which we discuss momentarily. 
\begin{enumerate}
\item Views on 1-hop queries, i.e., edges, that satisfy arbitrary predicates, such as transfers with \texttt{amount}$>$1000 USD or made to accounts with \texttt{balance} $>$ 5000. These are stored in {\em secondary vertex-partitioned A+ indexes}, which are partitioned primarily by vertex IDs.
\item Global views on 2-hop queries, i.e., 2-paths, are stored in {\em secondary edge-partitioned A+ indexes}, which are partitioned primarily by edge IDs.
\end{enumerate}

\noindent Edge-partitioned indexes extend the notion of adjacency %from vertices
to edges, which is highly beneficial for some applications.

\begin{example}
\label{ex:money-flow}
	Consider the following query, which is the core of an important class of queries in financial fraud detection.%\footnote{Informed by discussions with developers of GaussDB~\cite{gaussdb}, a system used by multiple financial institutions.}.
{\em
\begin{lstlisting}[numbers=none, mathescape=true, showstringspaces=false]
MATCH $a_1$$-$$[$$r_1$$:$$$$]$$-$$>$$a_2$$-$$[$$r_2$$:$$$$]$$-$$>$$a_3$$-$$[$$r_3$$:$$$$]$$-$$>$$a_4$
WHERE $r_1$$.$eID$=$$t13$$,$
$r_1$$.$$a$$m$$t$$>$$r_2$$.$$a$$m$$t$$,$ $r_1$$.$$a$$m$$t$$<$$r_2$$.$$a$$m$$t$ $+$$\;\alpha$$,$ $r_1$$.$$d$$a$$t$$e$$<$$r_2$$.$$d$$a$$t$$e$$,$
$r_2$$.$$a$$m$$t$$>$$r_3$$.$$a$$m$$t$$,$ $r_2$$.$$a$$m$$t$$<$$r_3$$.$$a$$m$$t$ $+$$\;\alpha$$,$ $r_2$$.$$d$$a$$t$$e$$<$$r_3$$.$$d$$a$$t$$e$
\end{lstlisting}
}
\noindent The query searches a three-step money flow path from a transfer edge with \texttt{eID t13} where each additional transfer (\texttt{Wire} or \texttt{Dir-Deposit}) happens at a later date and for a smaller amount of at most $\alpha$, simulating some money flowing through the network with intermediate hops taking cuts.
\end{example}

\begin{figure}[t!]
	\begin{subfigure}{0.47\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[scale=0.52]{images/indexes-vb}
		\vspace{-6pt}
		\caption{Example primary adjacency lists and secondary vertex-partitioned adjacency lists.}
		\label{fig:global-view}
	\end{subfigure}\vspace{2pt}
	\begin{subfigure}{0.47\textwidth}
		\centering
		\captionsetup{justification=centering}
		\includegraphics[scale=0.52]{images/indexes-eb}
		\vspace{-6pt}
		\caption{Example secondary edge-partitioned A+ Index.}
		\label{fig:global-view2}
	\end{subfigure}
	\caption{Example A+ indexes on our running example.}
\end{figure}

\noindent The predicates of this query compare properties of an edge on a path with the previous edge on the same path. Consider a system that matches r$_1$ to \texttt{t13}, which is from vertex \texttt{v2} to \texttt{v5}. Existing systems have to read transfer edges from \texttt{v5} and filter those that have a later \texttt{date} value than \texttt{t13} and also have the appropriate \texttt{amount} value.
Instead, when the next query edge to match r$_2$ has predicates depending on the query edge r$_1$, these queries can be  evaluated much faster if adjacency lists are partitioned by edge IDs:  a system can directly access the {\em forward adjacency list of} \texttt{t13}, i.e., edges whose \texttt{srcID} are \texttt{v5}, that satisfy the predicate on the \texttt{amount} and \texttt{date} properties that depend on \texttt{t13}, and perform the extension. Our edge-partitioned indexes allow the system to generate plans that perform this much faster processing.

\noindent {\bf Offset Lists:} 
Storing secondary A+ indexes requires data duplication and consumes extra memory. 
Our  approach to addressing the memory footprint of secondary indexes is based on two important observations: (1) each list in every secondary A+ index is a subset of some list in the primary A+ indexes, which is a result of our design of secondary indexes; and (2) each list in the primary A+ indexes contains a very small number of edges, which is a result of the sparsity, i.e., small average degrees, of real-world graphs. Therefore, 
instead of duplicating the globally identifiable (edge ID, neighbour ID) pairs that are stored in A+ indexes, secondary A+ indexes can store much smaller, often one or two byte, list-level identifiable pointers into the primary adjacency lists. We refer to lists of primary and secondary A+ indexes as {\em ID lists} and {\em offset lists}, respectively. Figures~\ref{fig:global-view} and~\ref{fig:global-view2} show examples of offset lists, for a secondary vertex-partitioned and an edge-partitioned A+ index, respectively. We demonstrate that secondary vertex-partitioned and edge-partitioned indexes can have very small memory overhead, as low as a few percentage points, making them highly practical. 

